Glitch in Time: Exploiting Temporal Misalignment of IMU For Eavesdropping

The increasing use of voice assistants and related applications has raised significant concerns about the security of Inertial Measurement Units (IMUs) in smartphones. These devices are vulnerable to acoustic eavesdropping attacks, jeopardizing user privacy. In response, Google imposed a rate limit of 200 Hz on permission-free access to IMUs, aiming to neutralize such side-channel attacks. Our research introduces a novel exploit, STAG, which circumvents these protections. It induces a temporal misalignment between the gyroscope and accelerometer, cleverly combining their data to resample at higher rates and reviving the potential for eavesdropping attacks previously curtailed by Google's security enhancements. Compared to prior methods, STAG achieves an 83.4% reduction in word error rate, highlighting its effectiveness in exploiting IMU data under restricted access and emphasizing the persistent security risks associated with these sensors.

==> devices.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{lm{1in}llllll}
\toprule
{\multirow{2}{*}{Device}} &
  {{Mean Freqs (Hz)}} &
  \multicolumn{2}{c}{Gyro Difference (ms)} &
  \multicolumn{2}{c}{Abs. Gyro Dev (ms)} &
  \multicolumn{2}{c}{Relative Gyro deviation (\%)} \\ \cmidrule(l){3-8} 
   & (acc-gyro)
   &
  {No Mag} &
  {With mag} &
  {No mag} &
  {With mag} &
  {No Mag} &
  {With Mag} \\ \midrule
Redmi Note 12 (2)      & 200.39-200.39 & 4.99   & 4.99   & 2.50   & 2.50   & 100.0000   & 100.0000   \\
Samsung Galaxy A72         & 206.57-206.57 & 3.72   & 3.72   & 1.30   & 1.30   & 53.7285    & 53.7284    \\
Redmi Note 11 (2)        & 202.94-202.95 & 4.36   & 4.36   & 1.89   & 1.89   & 76.8657    & 76.8516    \\
Samsung Galaxy A32 (3)        & 200.00-200.00 & 0.08   & 0.08   & 2.42   & 2.42   & 96.5593    & 96.2056    \\
Samsung Galaxy S20+        & 200.00-200.00 & 0.40   & 5.00   & 2.41   & 2.50   & 96.3397    & 99.9934    \\
Google Pixel 5          & 216.68-216.68 & 3.50   & 1.78   & 1.19   & 0.53   & 51.4633    & 22.9684    \\
Samsung Galaxy A54         & 121.62-121.62 & 0.09   & 0.08   & 4.03   & 4.03   & 97.7700    & 97.9920    \\
Samsung Galaxy A73 (5)        & 200.00-200.00 & 5.00   & 5.00   & 2.50   & 2.50   & 100.0000   & 100.0000   \\
ONEPLUS 6T    & 208.52-208.53 & 2.40   & 2.40   & 0.00   & 0.00   & 0.0093     & 0.0092     \\
Huawei Y9 Prime          & 251.86-251.86 & 0.85   & 0.85   & 1.13   & 1.13   & 57.1341    & 57.1340    \\
Samsung Galaxy A33 (3)        & 125.37-125.37 & 0.06   & 4.01   & 3.93   & 0.02   & 98.4629    & 0.5662     \\
OnePlus Nord CE           & 198.84-198.84 & 5.03   & 5.03   & 2.51   & 2.51   & 100.0000   & 100.0000   \\
Redmi Note 8     & 199.21-199.21 & 5.02   & 5.02   & 2.51   & 2.51   & 100.0000   & 100.0000   \\
vivo 1906        & 199.13-99.30  & 632.56 & 633.58 & 630.06 & 631.07 & 25093.0811 & 25131.9299 \\
Google Pixel 7 Pro (2)     & 454.38-454.38 & 2.20   & 2.20   & 1.10   & 1.10   & 100.0000   & 100.0000   \\
Redmi Note 8 Pro & 197.56-197.56 & 5.06   & 5.06   & 2.53   & 2.53   & 100.0000   & 100.0000   \\
Redmi Note 10 Pro (2)      & 203.30-203.30 & 3.80   & 3.80   & 1.34   & 1.34   & 54.4583    & 54.4600    \\
Samsung Galaxy M31         & 125.81-125.81 & 4.01   & 0.05   & 0.02   & 3.92   & 0.5797     & 98.7281    \\ \bottomrule
\end{tabular}
\end{table}

==> images/mainflow.tex <==
% % \section{Diagrammatic view of Multisketch operations}\label{app:mainflow}  

% % A user registers with a user id $\u$ and a vector of biometric templates
% % $\mvec=\mvecss{\mlen}$. Multisketch uses two databases $\dbid$ and $\dbmsg$\@,
% % where $\dbid$ contains user id $\u$ and the corresponding helper data
% % $\sketchval$, and $\dbmsg$ contains the random permutation of the templates
% % registered so far. Highlighted are the entries corresponding to a user $\u_4$
% % with templates $\mvec_4=\mvec_{41}\ldots\mvec_{4\mlen}$.% and helper
% %     % data $\sketchval_4$.
% \begin{figure}[t]
%   \centering
%   \begin{tikzpicture}[
%     >=stealth,
%     node distance=2cm,
%     database/.style={
%       cylinder,
%       cylinder uses custom fill,
%       cylinder body fill=black!25!white,
%       cylinder end fill=black!25!white,
%       shape border rotate=90,
%       aspect=0.25,
%       minimum width=2em,
%       minimum height=2em,
%       draw
%     },
%     func/.style={
%       rectangle,
%       fill=red!25!white,
%       minimum width=1cm,
%       minimum height=1em,
%       draw
%     },
%     cell/.style={
%       rectangle,
%       draw=black!50!white
%     }
%     ]
%     \node (user) at (0, 0) {User};
%     \node[func, right of=user, right=-1.1em, above=3em] (msketch) {$\MS$}; 
%     \draw[below of=msketch, dashed, anchor=west] (.85,0.55) rectangle (5.9,-1.2); 
%     \node[func, below of=msketch, anchor=east, below=1.95cm,fill=red!10!white,dashed] (mrecover) {$\MRec$};
%     % \node[database, right of=user, anchor=south, above=1em, right=2cm] (db1) {$\dbid$};
%     \matrix (db1) [right of=user, anchor=south, below=2pt, right=-0.1cm, 
%     matrix of math nodes,
%     column sep = -\pgflinewidth,
%     row sep=-\pgflinewidth,
%     column 1/.style={nodes={cell}}, 
%     column 2/.style={nodes={cell}}, 
%     anchor=west] {
%       \u_1 & \sketchval_1\\
%       \u_2 & \sketchval_2\\
%       \u_3 & \sketchval_3\\
%       |[draw,fill=blue!20]|\u_4 & |[draw,fill=blue!20]|\sketchval_4\\
%     };
%     \node[left of=db1, anchor=east,right=1.1cm] {$\dbid$};
%     \matrix (db2) [right of=db1, left=25pt, matrix of math nodes,
%     column sep = 2\pgflinewidth,
%     row sep=-\pgflinewidth,
%     column 1/.style={nodes={cell}},
%     column 2/.style={nodes={cell}}, 
%     column 3/.style={nodes={cell}}, 
%     column 4/.style={nodes={cell}}, 
%     column 5/.style={nodes={cell}}, 
%     anchor=west] {
%       \mvec_{21} &\mvec_{12} & |[draw,fill=blue!20]|\mvec_{43} &  & \mvec_{3\mlen} \\
%       |[draw,fill=blue!20]|\mvec_{41} &\mvec_{32} & \mvec_{33} & |[draw=white]|\ldots & \mvec_{2\mlen} \\
%       \mvec_{11} &|[draw,fill=blue!20]|\mvec_{42} & \mvec_{23} &  & \mvec_{1\mlen} \\
%       \mvec_{31} &\mvec_{22} & \mvec_{13} & & |[draw,fill=blue!20]|\mvec_{4\mlen} \\
%     };
%     \node[left of=db2, left=-4pt] {$\dbmsg$};

%     % \node[database,right of=db1] (db2) {$\dbmsg$};
%     \node[func,below of=db1,anchor=north,above=8pt,left=8pt] (gu) {GetUser};
%     \node[func,right of=gu,anchor=east,right=-5pt] (fm) {FindMatches};
%     \node[func,below of=db1,anchor=east,below=2em,right=-3pt] (recover) {Recover};

%     \draw[->,blue!50,thick] (user.north) |- node[black,near end,above]{$u, \mvec$} node[black,near end,below,font=\small]{register} 
%     (msketch.west);
%     \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$u, \sketchval$} (db1);
%     \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$\mvec$} (db2);

%     \draw[->,blue!50,thick] (user.south) |- ++(1,-0.9) node[black,near end,above]{$u, \mvectilde$} node[black,near end,below,font=\small]{login}   -| node[black,left,near end]{$u$}
%     (gu.north);
%     \draw[->,blue!50,thick] (user.south) |- ++(0,-0.9)  -- ++(3.1,0) |- node[black,near end, above]{$\mvectilde$}
%     (fm.west);
%     \draw[->,blue!50,thick] (db1.south) |- node[black,near end,above]{} (gu.east);
%     \draw[->,blue!50,thick] (db2.south) |- node[black,near end,above]{} (fm.east);
%     \draw[->,blue!50,thick] (gu.south) |- node[black,near end,above]{$\sketchval$} (recover.west);
%     \draw[->,blue!50,thick] (fm.south) |- node[black,near end,above]{$\mvec'$} (recover.east);    
%     \draw[->,blue!50,line width=2pt] (recover.south) -- node[black,near end,right]{$\mvec$ or $\bot$} ++(0, -0.65);
%   \end{tikzpicture}
%   % \rcnote{Rough sketch of the flow of the \biosketch.} 
%   \caption{Diagram of multisketch as a part of an authentication service. 
%   }
%   \label{fig:mainflow}
% \end{figure}

% %%% Local Variables:
% %%% mode: latex
% %%% TeX-master: "../main"
% %%% End:


==> mobiletable.tex <==
\begin{table*}[t]
\begin{tabular}{lllp{1in}p{1in}}
\toprule
 &
  \textbf{Model} &
  \textbf{Android Version} &
  \textbf{Before magnetometer ($ms$)} &
  \textbf{After magnetometer ($ms$)} \\ \midrule
\multicolumn{1}{c}{} & \cellcolor[HTML]{9AFF99}SM-A505F         & \cellcolor[HTML]{9AFF99}12 & \cellcolor[HTML]{9AFF99}-1.95 & \cellcolor[HTML]{9AFF99}0.03 \\
\multicolumn{1}{c}{} & \cellcolor[HTML]{9AFF99}SM-M315F         & \cellcolor[HTML]{9AFF99}12 & \cellcolor[HTML]{9AFF99}-1.94 & \cellcolor[HTML]{9AFF99}-0.01 \\
\multicolumn{1}{c}{\multirow{-3}{*}{Category A}} &
  \cellcolor[HTML]{9AFF99}SM-A515F &
  \cellcolor[HTML]{9AFF99}12 &
  \cellcolor[HTML]{9AFF99}2.50 &
  \cellcolor[HTML]{9AFF99}0.01 \\
                     & \cellcolor[HTML]{FFFC9E}Pixel 5          & \cellcolor[HTML]{FFFC9E}13 & \cellcolor[HTML]{FFFC9E}-0.53 & \cellcolor[HTML]{FFFC9E}-2.50 \\
                     & \cellcolor[HTML]{FFFC9E}Redmi Note 9 Pro & \cellcolor[HTML]{FFFC9E}12 & \cellcolor[HTML]{FFFC9E}0.00 & \cellcolor[HTML]{FFFC9E}2.50 \\
\multirow{-3}{*}{Category B} & \cellcolor[HTML]{FFFC9E}V2031            & \cellcolor[HTML]{FFFC9E}13 & \cellcolor[HTML]{FFFC9E}-0.09 & \cellcolor[HTML]{FFFC9E}2.50 \\
                     & \cellcolor[HTML]{FFCCC9}Infinix X680B    & \cellcolor[HTML]{FFCCC9}11 & \cellcolor[HTML]{FFCCC9}-2.50 & \cellcolor[HTML]{FFCCC9}2.50 $^1$ \\
                     & \cellcolor[HTML]{FFCCC9}LDN-L21          & \cellcolor[HTML]{FFCCC9}11 & \cellcolor[HTML]{FFCCC9}NA $^2$ & \cellcolor[HTML]{FFCCC9}NA \\
                     & \cellcolor[HTML]{FFCCC9}SM-A045F         & \cellcolor[HTML]{FFCCC9}12 & \cellcolor[HTML]{FFCCC9}NA $^3$ & \cellcolor[HTML]{FFCCC9}NA \\
                     & \cellcolor[HTML]{FFCCC9}SM-G973F         & \cellcolor[HTML]{FFCCC9}13 & \cellcolor[HTML]{FFCCC9}-2.50 & \cellcolor[HTML]{FFCCC9}2.49 \\
                     & \cellcolor[HTML]{FFCCC9}SM-A325F         & \cellcolor[HTML]{FFCCC9}13 & \cellcolor[HTML]{FFCCC9}-2.42 & \cellcolor[HTML]{FFCCC9}-2.42 \\
                     & \cellcolor[HTML]{FFCCC9}2201117TG        & \cellcolor[HTML]{FFCCC9}12 & \cellcolor[HTML]{FFCCC9}1.90 & \cellcolor[HTML]{FFCCC9}2.50 \\
\multirow{-8}{*}{Category C} &
  \cellcolor[HTML]{FFCCC9}SM-G950W &
  \cellcolor[HTML]{FFCCC9}13 &
  \cellcolor[HTML]{FFCCC9}-2.41 &
  \cellcolor[HTML]{FFCCC9}-2.41 \\
  \bottomrule
\end{tabular}\\
\hspace{-1.25in}{\footnotesize $^{1}$ The absolute difference matters here, therefore, not a significant change.}\\
\hspace{-2.25in}{\footnotesize $^{2,3}$ The device didn't have a working gyroscope sensor}\\[\baselineskip]
\label{tab:devices_eval}
\caption{Devices evaluation}
\end{table*}


==> reltable.tex <==
% \begin{tabular}{ | m{6em} | m{6em} | m{10em} | m{5em} | m{5em} | m{5em}|}
\begin{table*}[t]
\centering
\label{tab:relw}
\caption{Overview of the previous related works}
{
\begin{tabular}{p{0.86in}p{0.52in}p{1.5in}p{0.75in}p{1.20in}p{1.18in}}
\toprule
\textbf{Paper}  & \textbf{Sensor} & \textbf{Recognition} & \textbf{Evaluation Metric}  & \textbf{Accuracy\newline(permission-based)} & \textbf{Accuracy (permission-less)} \\
\midrule
Gyrophone \cite{184479} & Gyro & Digits (constrained) & Accuracy  & NA &  17\% \\
\midrule
Accelword \cite{10.1145/2742647.2742658} & Acc    & Words (constrained)    & F-measure & NA                   & 85\%                      \\
\midrule
PitchIn \cite{7944789}  & Acc    & Words (constrained)       & Accuracy & 79\%                      & NA                      \\
\midrule
Spearphone \cite{10.1145/3448300.3468499} &
  Acc &
  Digits + Words \newline(constrained) &
  F-measure &
  \begin{tabular}[c]{@{}l@{}}Digits: 71\%,\\ Words: 67\% \end{tabular} &
  NA \\
\midrule
AccelEve \cite{inproceedings-acceleve}& Acc & Digits + Letters \newline(constrained) & Accuracy & 55\% & NA \\
\midrule
AccEar \cite{9833716}  & Acc    & Words (unconstrained)      & 1-WER      & 80\%                      & NA                      \\
\midrule
InertiEar \cite{9796890} & Acc+Gyro & Digits + Letters \newline(constrained) & Accuracy & NA &78.8\%\\
\midrule
StealthyIMU \cite{inproceedings} & Acc & Spoken Language Understanding (unconstrained) & 1-SER & 87\% &37\%\footnote{This error rate was far larger in our testing}\\
\midrule
STAG [Ours] & Acc+Gyro & Spoken Language Understanding (unconstrained) & 1-SER \n 1-WER &  & 58 \n 93.5 \\

\bottomrule
\end{tabular} 
}
\end{table*}
